Resolving the Correct Library: A Loader-Level Defense Solution Against Shared Object Hijacking

Shared library hijacking attacks in the Linux ecosystem, including embedded Linux, are a significant concern. It fundamentally exploits the dynamic linker's library-resolution semantics rather than modifying trusted libraries directly. Prior research has extensively analyzed attack vectors exploiting environment variables, embedded search paths, and dynamic loader internals, demonstrating that hijacking is rooted in fundamental loader behavior rather than isolated misconfigurations. Existing defenses either harden or replace the loader, enforce control-flow integrity after libraries are loaded, or apply file-centric integrity mechanisms such as signatures and measurement frameworks. However, these approaches fail to address a critical gap: none verify whether the shared object actually resolved by the loader is the intended and trusted one. In this paper, we argue that shared library hijacking is fundamentally a loader-resolution authenticity problem and present a loader-centric verification framework that enforces authenticity guarantees for the dynamic linker's resolution process. Our design supports both path-bound and location-independent (i.e., Build-ID-based) identity models combined with cryptographic hashing. We implement our approach on GNU libc (glibc) systems and evaluate it on both general-purpose Linux (e.g., Ubuntu) and embedded Linux (e.g., Buildroot) environments under emulation. Our results demonstrate that our proposed mechanism indeed prevents shared library hijacking attacks.

==> Relationship_to_Software_Supply_Chain_Security.tex <==
\section{Relationship to Software Supply Chain Security}

Modern software supply-chain security mechanisms primarily focus on protecting the integrity and provenance of software artifacts during development, packaging, and distribution. Examples include signed packages, reproducible builds, Software Bill of Materials (SBOM) frameworks, and integrity verification systems such as IMA and fs-verity. These mechanisms help ensure that software components originate from trusted sources and have not been tampered with during delivery or installation.

However, shared library hijacking is a distinct class of threat that occurs at runtime during dynamic linking. In such attacks, adversaries do not necessarily modify trusted binaries or compromise the build pipeline itself. Instead, they manipulate the dynamic loader’s resolution process so that an unintended shared object is selected and loaded before the legitimate dependency. As a result, even correctly signed and authentic software packages may still be vulnerable if runtime library resolution can be influenced through search-path manipulation or unsafe loading semantics.

Our approach, therefore, complements existing software supply-chain protections. Supply-chain integrity mechanisms establish trust in distributed artifacts, whereas our mechanism enforces runtime authenticity of dynamically resolved shared objects after deployment. More specifically, the proposed loader-level verification ensures that only explicitly approved libraries can be resolved and mapped into the process address space, even if an attacker can place alternative libraries within the loader’s search scope.

This distinction is necessary because traditional integrity systems verify whether a library is authentic, but generally do not verify whether it is the correct library intended for a particular runtime dependency resolution event. By binding runtime-loaded shared objects to approved identities and cryptographic hashes, our mechanism constrains a class of post-deployment dependency substitution attacks that traditional supply-chain protections may not address.

It should be noted that our mechanism does not defend against all software supply chain attacks at the same time, for example, compromise of the trusted build environment itself. If an attacker successfully compromises the software supply chain prior to deployment—for example, by injecting malicious code into the build pipeline or producing malicious libraries that are subsequently signed and approved—then the loader-level verification process will still accept those artifacts. Therefore, our work should be viewed as a complementary runtime enforcement mechanism that strengthens post-deployment guarantees of dependency authenticity within a broader software supply-chain security architecture.

==> attack_surface_analysis.tex <==
\section{Static Binary Analysis of Shared Object Resolution Attack Surface}
\label{sec:binary-analysis-hijack-surface}

This section describes our static binary analysis approach for extracting the \emph{attack surface for shared object hijacking} from Linux ELF binaries using a Ghidra-based analysis plugin. The core premise is that shared object hijacking is primarily a \emph{resolution precedence} problem: if an attacker can introduce a malicious shared object with a matching name into a directory that the dynamic loader searches earlier than the intended location, the attacker-controlled code can be loaded into the target process. Consequently, our plugin focuses on identifying the binary- and loader-derived conditions that influence shared object resolution order, rather than attempting to prove exploitability in a specific deployment.

\subsection{Design Goals and Scope}

The plugin is designed to be \emph{binary-centric} and \emph{static}. The primary analysis target is a single ELF executable or shared object opened in Ghidra. The plugin extracts the metadata that governs how the runtime loader resolves dependencies, and reports \emph{conditions} under which hijacking becomes possible. Because feasibility depends on context (filesystem permissions, packaging, secure execution, etc.), the plugin avoids simplistic vulnerability labels and instead provides evidence for reasoning about hijack surface.

In addition to direct inspection of the opened ELF object, the plugin performs a bounded \emph{transitive dependency analysis} to capture hijacking surface introduced by dependencies. This analysis is configured via a user-supplied \emph{sysroot} that represents the filesystem context against which shared objects are resolved. The sysroot can be the host root directory (e.g., \texttt{/} on Ubuntu) or an extracted root filesystem (e.g., firmware rootfs, Buildroot target directory). To keep the analysis tractable while still capturing meaningful propagation of hijack surface, transitive resolution is limited to two dependency levels: the plugin resolves and analyzes (i) the direct dependencies of the root binary and (ii) the dependencies of those dependencies.

\subsection{Threat Model Alignment: What the Plugin Detects}

The plugin is aligned with a threat model in which the attacker’s capability is to influence the presence or placement of shared objects in one or more directories consulted by the loader. The plugin therefore aims to identify \emph{where precedence can be gained}, by detecting:

\begin{itemize}
  \item \textbf{Hijack targets:} shared object names that must be resolved at load time (and thus can be substituted if precedence is obtained).
  \item \textbf{Precedence mechanisms:} embedded search paths (RPATH/RUNPATH), origin-relative resolution (\texttt{\$ORIGIN}), and default resolution directories implied by the platform.
  \item \textbf{Propagation paths:} whether dependencies introduce additional search paths (and thus additional hijack surface) transitively.
  \item \textbf{Loader context signals:} the interpreter specified by \texttt{PT\_INTERP}, which indicates the loader family and provides context for search-order interpretation.
\end{itemize}

The plugin does not claim that hijacking will occur. Instead, it enumerates \emph{necessary conditions} for hijacking (e.g., ``a library named \texttt{libX.so} is resolved from an origin-relative directory''), leaving environment-specific feasibility (e.g., directory write permissions) to be handled explicitly in later methodological steps.

\subsection{Extracted ELF Properties and Their Relevance}

Shared object hijacking is governed by a small set of ELF constructs that determine (i) which shared objects are required and (ii) which locations are searched to satisfy those requirements. The plugin extracts and reports the following properties.

\subsubsection{Dynamic Loader Identification (PT\_INTERP)}

The plugin extracts the interpreter path specified by the \texttt{PT\_INTERP} program header (e.g., \texttt{/lib64/ld-linux-x86-64.so.2}). This is a critical contextual artifact because the dynamic loader implementation determines the exact semantics of shared object search order and environment handling. The interpreter path is therefore reported as part of the evidence for interpreting precedence-related findings.

\subsubsection{Direct Dependency Targets (DT\_NEEDED)}

The plugin enumerates all \texttt{DT\_NEEDED} entries in the ELF dynamic table. Each \texttt{DT\_NEEDED} string is a shared object name that must be resolved by the loader. These names define the primary hijack targets because an attacker can substitute a malicious shared object if they can place it earlier in the resolution order. Reporting the full list of \texttt{DT\_NEEDED} entries also supports downstream analyses such as identifying unversioned or generic names that may be easier to impersonate in practice.

\subsubsection{Embedded Search Paths (DT\_RPATH and DT\_RUNPATH)}

The plugin extracts embedded search paths specified via \texttt{DT\_RPATH} and \texttt{DT\_RUNPATH}. These tags encode directory lists that influence the loader’s search order. From a hijacking perspective, any non-system directory introduced into the search sequence can become a placement opportunity for an attacker, depending on filesystem controls. The plugin reports both tags separately because they reflect different linking conventions and can have different precedence behavior in loader implementations.

\subsubsection{Origin-Relative Resolution (\texttt{\$ORIGIN})}

The plugin detects the use of \texttt{\$ORIGIN} (and \texttt{\$\{ORIGIN\}}) within RPATH/RUNPATH entries. Origin-relative paths are widely used to support relocatable deployment (e.g., bundling an executable and its libraries). However, origin-relative directories can create hijack surface if an attacker can write to or influence the path surrounding the binary (e.g., writable installation directories, insecure extraction locations). The plugin flags \texttt{\$ORIGIN} explicitly because it indicates a strong coupling between filesystem layout and resolution precedence.

\subsection{Implementation Strategy in Ghidra}

To ensure robustness and reproducibility, the plugin parses ELF metadata directly from the original file bytes rather than relying only on higher-level framework abstractions that may vary across versions or differ between the file layout and the imported memory view. The plugin reads the ELF identification bytes to determine the file class and endianness, parses the ELF header and program headers, and then extracts relevant information from the interpreter and dynamic segments.

\subsubsection{Parsing the ELF File Layout}

The plugin first validates the ELF magic and then parses:

\begin{itemize}
  \item the ELF header to locate the program header table,
  \item program headers to locate \texttt{PT\_INTERP} and \texttt{PT\_DYNAMIC},
  \item the dynamic tag array (\texttt{ElfXX\_Dyn}) to enumerate \texttt{DT\_NEEDED}, \texttt{DT\_RPATH}, \texttt{DT\_RUNPATH}, and the string table pointers (\texttt{DT\_STRTAB}, \texttt{DT\_STRSZ}).
\end{itemize}

Dynamic entries provide offsets into the dynamic string table. The plugin resolves these offsets to concrete strings (dependency names and path lists). This produces a loader-relevant description of the binary’s shared object resolution behavior independent of any runtime execution.

\subsection{Two-Level Transitive Dependency Analysis with Sysroot}

A key challenge in characterizing hijacking surface is that dependencies can introduce additional surface. For example, even if the main executable does not embed a risky search path, a dependent shared object may embed origin-relative search paths, thereby expanding the set of directories in which a malicious library could gain precedence. To capture this phenomenon, the plugin performs a bounded transitive analysis.

\subsubsection{Sysroot Configuration}

The plugin prompts the analyst for a sysroot path. The sysroot represents the filesystem that should be used to resolve dependencies during analysis. On a desktop system, selecting \texttt{/} approximates the host environment. For embedded studies, selecting an extracted root filesystem (e.g., firmware rootfs directory) enables analysis consistent with the device’s library layout. By making sysroot explicit, the plugin avoids implicit assumptions about where libraries are located and supports consistent evaluation across environments.

\subsubsection{Resolution Heuristic and \texttt{\$ORIGIN} Expansion}

When resolving a dependency name (e.g., \texttt{libc.so.6}), the plugin consults:

\begin{enumerate}
  \item Embedded RPATH/RUNPATH entries of the owning object, after expanding \texttt{\$ORIGIN} relative to that object’s directory.
  \item A set of standard library directories under the sysroot (e.g., \texttt{/lib}, \texttt{/usr/lib}, and architecture-specific subdirectories).
\end{enumerate}

This resolution heuristic is intentionally conservative and designed for attack-surface characterization: it aims to locate the concrete library file that would plausibly satisfy a \texttt{DT\_NEEDED} entry in the given sysroot, thereby enabling further inspection of that library’s own dependency and path metadata.

\subsubsection{Bounded Dependency Closure}

The plugin applies the same ELF parsing pipeline to each resolved dependency at level~1, extracts its \texttt{DT\_NEEDED} entries and embedded paths, and then resolves those dependencies at level~2. A visited set prevents cycles and repeated analysis. Limiting depth to two balances coverage and tractability while capturing common real-world propagation (e.g., executable $\rightarrow$ vendor library $\rightarrow$ libc/loader).

\subsection{Output: Evidence for Hijacking Attack Surface}

The plugin produces a structured report that includes:

\begin{itemize}
  \item The root ELF object’s interpreter (\texttt{PT\_INTERP}), direct dependencies (\texttt{DT\_NEEDED}), and embedded search paths (RPATH/RUNPATH), with explicit \texttt{\$ORIGIN} flags.
  \item A two-level dependency tree where each resolved shared object is annotated with its own \texttt{DT\_NEEDED} set and embedded search paths.
  \item Unresolved dependencies, which indicate missing libraries in the sysroot or non-standard layouts and may themselves be relevant signals for deployment-specific resolution behavior.
\end{itemize}

This output enables analysts to identify (i) which shared object names are hijack targets, (ii) which path mechanisms introduce precedence opportunities (especially origin-relative paths), and (iii) whether hijack surface originates in the main binary or is introduced transitively by dependencies.

\subsection{Summary}

Our Ghidra plugin statically extracts shared object hijacking attack surface by focusing on the relationship between dependency names and loader search precedence. By parsing ELF interpreter and dynamic metadata directly from file bytes and extending the analysis transitively under a configurable sysroot, the plugin provides a repeatable foundation for identifying where attacker-controlled shared objects could gain precedence in the resolution order. This analysis serves as an evidence-producing measurement instrument for subsequent prevention and deterrence methodology design.


==> attack_surface_analysis_v2.tex <==
\section{Static Binary Analysis for Hijacking Attack Surface}
\label{sec:binary-analysis-hijack-surface}

%In this section, we address the challenge that shared object hijacking lacks a systematic, static method for identifying the attack surface at the binary level. While hijacking attacks are well known, existing analyses typically rely on dynamic execution, exploit demonstrations, or environment-specific reasoning, making results difficult to reproduce or compare. The research challenge we address is to characterize shared object hijacking surface directly from ELF binaries by extracting the resolution-precedence conditions encoded in the binary and its dependencies. Our Ghidra-based analysis provides a binary-centric and reproducible way to expose where and how attacker-controlled shared objects could gain precedence in the dynamic loader’s search order, without asserting exploitability or relying on runtime behavior.

%To address this gap, we developed a static analysis plugin for Ghidra that characterizes the \emph{shared object hijacking attack surface} of Linux ELF binaries. The goal of the plugin is not to determine whether a binary is exploitable in a particular deployment, but to expose the binary-level conditions under which hijacking becomes possible. In this context, the attack surface is defined as the set of shared object names and resolution paths for which an attacker-controlled library could gain precedence over the intended dependency.

A common approach to inspecting shared library dependencies on Linux systems is the use of the \texttt{ldd} utility. Given an ELF binary, \texttt{ldd} reports the shared objects that are resolved when the binary is executed under the current environment. While useful for runtime diagnostics, this approach has fundamental limitations when applied to the analysis of shared object hijacking.

First, \texttt{ldd} is inherently dynamic and environment-dependent. Its output reflects a single resolution outcome under the current filesystem layout, loader configuration, and environment variables. If a malicious shared object is not present at analysis time, \texttt{ldd} provides no indication that hijacking would be possible under a different placement or deployment scenario. As a result, \texttt{ldd} cannot capture potential resolution-precedence conditions, which are central to shared object hijacking.

Second, \texttt{ldd} collapses resolution semantics into a final result. It reports which shared object was loaded, but not \emph{why} it was selected or which alternative search paths were considered earlier in the resolution order. Therefore, mechanisms such as \texttt{DT\_RPATH}, \texttt{DT\_RUNPATH}, and origin-relative resolution via \texttt{\$ORIGIN} are not exposed as attack surface, even though they define where attacker-controlled libraries could gain precedence.

Third, \texttt{ldd} provides limited insight into the transitive hijacking surface. Although it lists dependencies of the root binary, it does not systematically expose how dependent shared objects introduce additional search paths or resolution behavior that may expand the hijacking surface beyond the main executable. Moreover, since \texttt{ldd} executes the dynamic loader, it is unsuitable for analyzing untrusted binaries and is difficult to apply consistently across embedded or non-native environments.

These limitations are not specific to \texttt{ldd} alone, but are shared by a broader class of dynamic or execution-based dependency inspection tools. Such tools are designed to answer the question of \emph{what is loaded in a specific environment}, whereas shared object hijacking requires reasoning about \emph{where precedence could be gained if the environment were manipulated}.

One may argue that static utilities such as \texttt{readelf}, \texttt{objdump}, and \texttt{nm} already expose the ELF metadata required to reason about shared object hijacking. Indeed, these tools provide faithful, specification-level access to dependency declarations, embedded search paths, symbol tables, and dynamic linking structures. In principle, this information is sufficient for an \textit{expert analyst} to reason about loader behavior.

However, these utilities are fundamentally descriptive. They simply report individual ELF fields without interpreting their security implications or modeling how they influence shared object resolution precedence. In particular, they do not explain how embedded mechanisms such as \texttt{DT\_RPATH}, \texttt{DT\_RUNPATH}, or origin-relative resolution via \texttt{\$ORIGIN} affect the loader’s search order, nor do they explicitly relate these mechanisms to potential hijacking attack surface. As a result, identifying hijacking conditions requires substantial manual effort and external knowledge of dynamic loader semantics.

Moreover, static inspection tools operate strictly on individual binaries. They provide no support for systematic transitive reasoning across dependency graphs, requiring analysts to manually inspect and correlate multiple executables and shared objects. Hijacking surface introduced indirectly by dependent libraries therefore remains difficult to identify, particularly in complex software stacks or embedded systems.

To address this gap, we developed a static, binary-centric analysis implemented as a Ghidra plugin. Rather than executing the binary, the plugin extracts the resolution mechanisms encoded directly in ELF metadata. Specifically, it identifies the dynamic loader, enumerates required shared object names, and extracts embedded search paths specified via \texttt{DT\_RPATH} and \texttt{DT\_RUNPATH}, with explicit detection of origin-relative resolution. These elements collectively define the resolution-precedence conditions that enable shared object hijacking, and they show two levels of transitive dependencies in the tree form.

A key design choice is the inclusion of bounded transitive dependency analysis. The plugin resolves dependencies under a user-specified sysroot representing the intended execution environment and applies the same extraction process to dependent shared objects. This makes it possible to identify hijacking surface that is introduced transitively, rather than directly by the root binary. By limiting the analysis depth, the approach remains tractable while capturing the most common propagation patterns observed in practice.

Importantly, the plugin does not claim exploitability. Its output should be interpreted as a characterization of the necessary conditions for shared object hijacking, independent of deployment-specific factors such as file system permissions. The analysis provides a reproducible and systematic basis for reasoning about the shared object hijacking attack surface by separating binary-encoded resolution semantics from environment-specific assumptions.


\subsection{Extracting Resolution-Relevant Binary Properties}

The plugin extracts ELF metadata that directly governs how the dynamic loader resolves shared objects. First, it identifies the dynamic loader specified by the \texttt{PT\_INTERP} program header. The interpreter path provides essential context for interpreting resolution semantics, as loader behavior differs across implementations and platforms.

Second, the plugin enumerates all \texttt{DT\_NEEDED} entries from the ELF dynamic table. These entries specify the shared object names that must be resolved at load time and therefore define the primary targets for hijacking. From an attacker’s perspective, each required name represents a potential substitution point if resolution precedence can be influenced.

Third, the plugin extracts embedded search paths specified via \texttt{DT\_RPATH} and \texttt{DT\_RUNPATH}. These paths directly affect the loader’s search order and are a common source of hijacking surface, particularly when they reference non-system directories. The plugin explicitly detects the use of \texttt{\$ORIGIN}, as origin-relative resolution ties dependency loading to filesystem layout and frequently appears in relocatable software bundles and embedded deployments. The presence of \texttt{\$ORIGIN} is treated as a strong indicator of location-dependent hijacking surface.

\subsection{Transitive Dependency Analysis Under a Sysroot}

A central observation motivating our design is that hijacking surface is not necessarily introduced by the main executable itself. Dependent shared objects may embed their own search paths, thereby expanding the overall resolution surface transitively. To capture this effect, the plugin performs a bounded transitive dependency analysis.

The analyst provides a \emph{sysroot} that represents the filesystem context in which dependencies should be resolved. On desktop systems, the sysroot can be the host root directory (e.g., \texttt{/}), while for embedded systems it may correspond to an extracted root filesystem. Using this sysroot, the plugin resolves each \texttt{DT\_NEEDED} entry by consulting embedded RPATH/RUNPATH directories (with \texttt{\$ORIGIN} expansion) followed by standard library locations under the sysroot.

Each resolved dependency is parsed using the same ELF analysis pipeline, and its own dependencies and embedded paths are extracted. This process is repeated for one additional level, yielding a two-level dependency closure. The depth is intentionally limited to balance analysis tractability with practical coverage, as most resolution-relevant propagation occurs within the first few dependency layers. A visited set prevents cycles and redundant analysis.

\subsection{Identifying Hijacking Attack Surface}

The plugin produces a dependency tree annotated with resolution-relevant metadata at each node. For the root binary and each resolved dependency, the output includes the dynamic loader, required shared object names, embedded search paths, and the presence of origin-relative resolution. This structure enables analysts to distinguish between hijacking surface introduced directly by the main binary and surface introduced transitively by dependent shared objects.

Importantly, the plugin does not claim that hijacking will occur in the analyzed environment. Instead, it enumerates the \emph{conditions} under which attacker-controlled shared objects could gain precedence in the loader’s search order. By making resolution paths and dependency propagation explicit, the analysis provides the necessary evidence for reasoning about hijacking feasibility in subsequent methodological steps.

Therefore, our Ghidra plugin statically characterizes the shared object hijacking attack surface by extracting dependency names and resolution precedence mechanisms from ELF binaries and their transitive dependencies. By combining direct binary inspection with bounded dependency resolution under an explicit filesystem context, the analysis reveals how hijacking surface emerges and propagates across shared object boundaries. This binary-level characterization forms the foundation for the prevention and deterrence methodology presented in the following section.


\subsection{Illustrative Example}
\label{subsec:illustrative-example}

In this subsection, we illustrate the output produced by our Ghidra plugin and demonstrate that it correctly extracts the shared object hijacking attack surface as intended. Figure~\ref{fig:ghidra-hijack-output} shows the analysis result for a dynamically linked ELF executable compiled with an origin-relative runtime search path.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/ghidra_output.png}
    \caption{Example output of the Ghidra-based shared object hijacking analysis.}
    \label{fig:ghidra-hijack-output}
\end{figure}

Figure~\ref{fig:ghidra-hijack-output} shows an example of the output produced by our Ghidra plugin when analyzing a dynamically linked ELF executable. The root binary embeds a \texttt{DT\_RUNPATH} entry containing \texttt{\$ORIGIN/lib}, indicating that the dynamic loader will search an origin-relative directory before consulting system library paths. This establishes a resolution-precedence condition under which an attacker-controlled shared object could be loaded if placed in the corresponding directory.

The analysis resolves direct dependencies of the root binary and propagates the inspection transitively. In this example, \texttt{libhello.so} is resolved from the origin-relative directory, and \texttt{libc.so.6} is resolved from a system-managed location. Subsequent dependencies do not introduce additional search paths.


==> notes.tex <==
Mode 1: Single-binary analysis (default, always available): The proposed Ghidra plugin performs static analysis of individual ELF binaries to identify potential shared library hijacking vectors based on dynamic linking metadata and dynamic loading patterns.

The dynamic loader’s resolution policy ultimately governs shared library hijacking, and differences between loaders materially affect both exploitability and mitigation effectiveness. Therefore, loader behavior must be explicitly modeled and evaluated.

A loader profile captures the shared library resolution semantics implemented by a specific dynamic loader (e.g., glibc, musl), including search order, configuration mechanisms, and environment variable handling.

Because shared library resolution semantics are implemented by the dynamic loader rather than the application, this work explicitly considers loader behavior as a first-class factor when analyzing shared library hijacking in embedded Linux systems.

Sign vs hash

normally, you can trace which shared objects are loaded via the strace utility. If that directory is writable, you can inject your own .so file. If the binary is suid, this gives you a root shell.

Is glibc hijackable? 

Security analysis of Buildroot, OpenWRT, including SELinux usage and ASLR presence.

If you use sudo and set the environmental variable LD\_LIBRARY\_PATH, you may encounter an issue because most modern operating systems do not pass user-level environmental variables. This behavior is controlled by the 'env\_rest' setting in the '/etc/sudoers'. To be able to overcome this issue, one can use a simple trick. Create an alias for sudo that includes the LD\_LIBRARY\_PATH variable.

alias sudo='sudo LD\_LIBRARY\_PATH=...'

Are OpenWrt and Buildroot installed with sudo by default?

Ubuntu 24.04 uses the GNU C Library (glibc) as its system C library, with the dynamic loader ld-linux-x86-64.so.2

Plugin
Which ELF-level properties introduce shared object hijacking surface?

How does loader behavior (glibc vs musl) change that surface?

How much hijack surface exists in real-world binaries and embedded firmware?

Can we identify hijack surface without executing code or knowing deployment context?

IMA does not automatically update reference hashes on reboot. Hash values are modified only when the system is booted in appraisal “fix” mode or during explicit provisioning steps; in enforcement mode, hashes remain immutable and any deviation results in denial of execution or library loading. If hashes ever update themselves during normal operation, the system is misconfigured.

We enforce DSO integrity for application DSOs and for any DSOs resolved from writable/untrusted locations (e.g., /tmp), while excluding baseline system components (dynamic loader, libc) from the LD\_AUDIT prototype to keep the allowlist minimal and portable.

Buildroot can be configured with either musl or glibc, which can be chosen at configuration time.

==> surface_analysis.tex <==
\section{Static Binary Analysis for Hijacking Attack Surface}
\label{sec:binary-analysis-hijack-surface}

Shared object hijacking arises from the resolution-precedence rules used by the dynamic loader when selecting shared libraries at runtime. A common approach to inspecting shared library dependencies on Linux systems is the use of the \texttt{ldd} utility, which reports the shared objects resolved when a binary is executed under a specific environment. However, this approach has fundamental limitations when applied to the systematic analysis of shared object hijacking.

First, \texttt{ldd} is inherently dynamic and environment-dependent. Its output reflects a single resolution outcome under the current filesystem layout, loader configuration, and environment variables. If a malicious shared object is not present at analysis time, \texttt{ldd} provides no indication that hijacking would be possible under a different placement or deployment scenario. As a result, it cannot capture potential resolution-precedence conditions, which are central to shared object hijacking. Second, \texttt{ldd} collapses resolution semantics into a final result: it reports which library was loaded, but not why it was selected or which alternative search paths were considered earlier in the resolution order. Consequently, mechanisms such as \texttt{DT\_RPATH}, \texttt{DT\_RUNPATH}, and origin-relative resolution via \texttt{\$ORIGIN} are not exposed as attack surface, even though they directly define where attacker-controlled libraries could gain precedence. Finally, since \texttt{ldd} executes the dynamic loader, it is unsuitable for analyzing untrusted binaries and difficult to apply consistently in embedded or non-native environments.

On the other hand, one may argue that static utilities such as \texttt{readelf}, \texttt{objdump}, and \texttt{nm} already expose the ELF metadata required to reason about shared object hijacking. Indeed, these tools provide specification-level access to dependency declarations, embedded search paths, symbol tables, and dynamic linking structures. In principle, this information is sufficient for an expert analyst to reason about loader behavior. However, these utilities are fundamentally descriptive. They report ELF fields in isolation without interpreting their security implications or modeling how they influence resolution precedence. Moreover, they operate strictly on individual binaries and provide no support for systematic \textit{transitive} reasoning (suppose that binary1 needs lib1 and lib1 needs lib2; in this case, lib2 is transitive) across dependency graphs. As a result, identifying hijacking surface, particularly when introduced indirectly by dependencies, requires substantial manual effort and deep external knowledge of loader semantics.

To address these limitations, we developed a static, binary-centric analysis implemented as a Ghidra plugin. The plugin extracts resolution-relevant mechanisms encoded directly in ELF metadata without executing them. Specifically, it identifies the dynamic loader specified by \texttt{PT\_INTERP}, enumerates required shared object names via \texttt{DT\_NEEDED}, and extracts embedded search paths specified through \texttt{DT\_RPATH} and \texttt{DT\_RUNPATH}, with explicit detection of origin-relative resolution. These elements collectively define the resolution-precedence conditions under which shared object hijacking becomes possible.

A central design choice is the inclusion of bounded two-level transitive dependency analysis. In some instances, the main executable does not necessarily introduce a hijacking surface; dependent shared objects may embed their own search paths, thereby expanding the overall resolution surface. The plugin resolves dependencies under a user-specified sysroot representing the intended execution environment, such as the host root directory or an extracted embedded root filesystem. Each resolved dependency is analyzed using the same extraction process, and its dependencies are inspected to a bounded depth. Limiting the analysis depth preserves tractability while capturing the most common propagation patterns observed in practice.

The output of the analysis is a structured dependency tree annotated with resolution-relevant metadata at each node, including required shared object names, embedded search paths, and the presence of origin-relative resolution. This structure enables analysts to distinguish between hijacking surfaces introduced directly by the root binary and those introduced transitively by dependent shared objects. Moreover, the plugin does not claim exploitability. Instead, its output should be interpreted as a characterization of the necessary conditions for shared object hijacking, independent of deployment-specific factors, such as file system permissions. Therefore, the analysis provides a reproducible and systematic basis for reasoning about the shared object hijacking attack surface.

\subsection{Illustrative Example}
\label{subsec:illustrative-example}

Figure~\ref{fig:ghidra-hijack-output} illustrates the output produced by our Ghidra plugin for a dynamically linked ELF executable compiled with an origin-relative runtime search path. The root binary embeds a \texttt{DT\_RUNPATH} entry containing \texttt{\$ORIGIN/lib}, indicating that the dynamic loader will search an origin-relative directory before consulting system-managed library paths. This establishes a resolution-precedence condition under which an attacker-controlled shared object could be loaded if placed in the corresponding directory.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/ghidra_output.png}
    \caption{Example output of the Ghidra-based shared object hijacking analysis.}
    \label{fig:ghidra-hijack-output}
\end{figure}

The analysis resolves direct dependencies of the root binary and continues the inspection transitively under the specified sysroot. In this example, a project-specific library is resolved from the origin-relative directory, while system libraries are resolved from standard locations. Dependent shared objects introduce no additional search paths. This illustrates how hijacking the surface can be localized to specific points in the dependency graph. This example demonstrates that the plugin correctly extracts and contextualizes resolution-precedence conditions without asserting exploitability, enabling systematic reasoning about shared object hijacking.


==> threat_model.tex <==
\section{Threat Model and Assumptions}
This work considers an attacker model commonly seen in embedded Linux deployments, where devices execute dynamically linked ELF binaries with minimal runtime isolation. The attacker is assumed to have non-kernel-level access to the target system, which may arise through local shell access, exploitation of a network-facing service, insecure update mechanisms, or physical access to device storage. Kernel compromise and hardware-backed trust mechanisms are explicitly out of scope.

The attacker’s primary capability is the ability to modify the filesystem within at least one writable directory that is reachable — directly or indirectly — by the dynamic loader during shared library resolution. Such writable locations may include application directories, update or plugin paths, writable overlays (e.g., /overlay, /data, or /opt), temporary directory (/tmp), or misconfigured library directories. The attacker is not assumed to have the ability to modify the target executable itself, nor to alter kernel memory or loader binaries.

The target binaries are dynamically linked user-space applications or services that rely on the dynamic loader to resolve shared object dependencies at runtime. These binaries may specify library search paths using DT\_RPATH or DT\_RUNPATH, depend on relative resolution via \$ORIGIN, or dynamically load shared objects through interfaces such as dlopen(). In many embedded Linux systems, these applications execute with elevated privileges, often as the root user, and without utilizing traditional desktop Linux privilege separation mechanisms.

The dynamic loader is treated as a trusted component whose behavior defines the effective library resolution policy. However, this work assumes no modifications to the loader itself; instead, the attacker exploits the loader’s intended resolution semantics in combination with filesystem and build-system choices. Differences in loader implementations (e.g., glibc versus musl), configuration mechanisms, and default search paths are therefore considered first-class factors influencing attack feasibility.

Environmental controls, such as LD\_LIBRARY\_PATH and LD\_PRELOAD, are included in the threat model only to the extent that they are honored by the loader in the evaluated configuration. Scenarios involving setuid or setgid binaries are not a primary focus, as many embedded systems operate without such privilege boundaries or execute all services as root. Network-based injection of shared objects, kernel-level rootkits, and runtime binary patching are excluded from consideration.

Under this threat model, a shared library hijacking attack is considered successful if the attacker can cause the dynamic loader to resolve and execute a malicious shared object in place of, or in addition to, an intended library, thereby achieving arbitrary code execution within the context of the target application. The proposed analyses and mitigation strategies are evaluated against this attacker model, with a particular emphasis on loader behavior and file system trust boundaries.

